Beyond Denouncing Hate: Strategies for Countering Implied Biases and Stereotypes in Language

Counterspeech, i.e., responses to counteract potential harms of hateful speech, has become an increasingly popular solution to address online hate speech without censorship. However, properly countering hateful language requires countering and dispelling the underlying inaccurate stereotypes implied by such language. In this work, we draw from psychology and philosophy literature to craft six psychologically inspired strategies to challenge the underlying stereotypical implications of hateful language. We first examine the convincingness of each of these strategies through a user study, and then compare their usages in both human- and machine-generated counterspeech datasets. Our results show that human-written counterspeech uses countering strategies that are more specific to the implied stereotype (e.g., counter examples to the stereotype, external factors about the stereotype's origins), whereas machine-generated counterspeech uses less specific strategies (e.g., generally denouncing the hatefulness of speech). Furthermore, machine-generated counterspeech often employs strategies that humans deem less convincing compared to human-produced counterspeech. Our findings point to the importance of accounting for the underlying stereotypical implications of speech when generating counterspeech and for better machine reasoning about anti-stereotypical examples.

==> emnlp2023-latex/content/qualitative-analysis.tex <==
\begin{table*}[]
    \centering
    \small
    \begin{tabularx}{\textwidth}{p{\textwidth}}
        \toprule
        Title: Gay men are incapable of a committed loving, monogamous relationship. CMV\\
        Implied Stereotype: Gay men cannot have committed, loving, monogamous relationships\\
        Post: This is from my personal anecdotal experiences. There are exceptions, but 98\% of gay men prefer a lifestyle of casual, multiple sexual relationships. A partial cause of this is the trauma of being marginalized and demonized by society; but given the choice and freedom to choose, a gay man will overwhelmingly choose a lifestyle of multiple partners over a monogamous committed relationship. I support gay marriage, but our portrayal of a gay family unit is a rarity from what is actually happening, statistically\\
        \midrule
        % \hline\\[-4ex]
        % \vspace{1mm}
        % \faCaretSquareUp[regular]\xspace 
        $\bm{\Delta}$ I'll just chime in on a similar note to others. If you're view is based on anecdotal experience, you should be swayed by the anecdotal experiences of others. \hlc[lightblue!40]{I've met lots of gay people, but most of them I honestly don't know what their sexual lifestyle is.} \hlc[lightblue!40]{But the two close gay friends I have are *both* in long-term monogamous relationships.} \hlc[lightblue!40]{Meanwhile, I know lots of heterosexual friends who at least at this point in their lives seem entirely disinterested in a long term monogamous relationship.} So my experiences seem to refute your position.\textbackslash n\textbackslash nIn addition, may I ask how you know the gay people you know? \hlc[lightblue!40]{If I went to a gay bar, I'd probably find a lot of gay people who are just looking for casual sex, but that's true of straight people who go to bars too...} \hlc[lightblue!40]{so watch out for confirmation bias.}\\
        \\[-2ex]
        % \faCaretSquareDown[regular]\xspace
        $\bm{\nabla}$ Of course my evidence is only anecdotal, but \hlc[lightapricot!40]{I am gay and have been in a committed monogamous relationship for 17 years.} That is the longest term relationship in my family, including immediate family who have all been married at least there times. I am also part of several gay themes meetups and am,active in several gay organizations, in all instances, \hlc[lightapricot!40]{majority of men are partnered and most of those relationships are a decade if not decades long.}\textbackslash n\textbackslash nAlso, of course you admitted this. \hlc[lightapricot!40]{It is wildly unfair to judge gay people by criteria that they are not permitted to engage in, namely marriage.}\\
        \\[-2ex]
        \faRobot\xspace While I understand that you're sharing your personal anecdotal experiences, \hlc[lavendergray!40]{it's important not to generalize the experiences and preferences of an entire group based on individual cases}. \hlc[lavendergray!40]{The preferences and choices of individuals within the LGBTQ+ community are as diverse as those in any other community.} \hlc[lavendergray!40]{It's crucial to recognize that people's choices and lifestyles are influenced by various factors, and it's not fair to assume that one's sexual orientation is the primary determinant of their relationship preferences.}\textbackslash n\textbackslash nMoreover, \hlc[lavendergray!40]{using a percentage like "98\%" without any supporting data or research can be misleading and perpetuate harmful stereotypes.} It's essential to remember that people's choices and preferences are personal and should not be used to judge or define an entire community. Instead, \hlc[lavendergray!40]{let's promote understanding, acceptance, and respect for everyone's individual choices and lifestyles, irrespective of their sexual orientation}.\\
        \bottomrule
    \end{tabularx}
    \caption{Examples of responses for comparison. Highlights were added to example quotes chosen by GPT-4 during each counter strategy labeling task. \jimin{will add specific labels to the highlights later}\jimin{a bit long - Xuhui suggests moving to the appendix}}
    % \maarten{is this missing the actual post?} \maarten{ Also replace "implied generic" with implied stereotype?}
    \label{tab:qualitative}
\end{table*}
% while this is a fitting example, I feel like I am publicly outing someon? Ask Maarten

\section{Qualitative Analysis}
\maarten{I would probably just move this entire section to the appendix, and try to add one sentence to the results that points to this section / Table 4 saying "qualitative analyses (\S\ref{}) show/confirm/suggest that ...}
In Table~\ref{tab:qualitative} we show one example of a harmful post from our Reddit dataset. 
The original post, which claims that ``gay men are incapable of a committed relationship'', and its implication that, ``gay men are promiscuous'', is countered by community members with counter examples.
However, GPT-4's repsonse is characterized by longer and frequent denouncing statements and lack of countering examples.
Moreover, the broadening method used and labelled by GPT-4 does not actually counter the implication but rather sets the tone (e.g., ``let's promote understanding [...] for everyone's individual choices''). 

Across a number of samples, we observe some common patterns in the usage of countering strategies. 
First, \den has higher occurrence in the beginning or end of the countering posts and is often supplemented with \cntrExs or \external descriptions as supporting evidence. Additionally, many \cntrExs are from first person experiences (e.g., ``my gay friends'') or the use of second person pronouns (e.g., ``you'd get made fun of'').
% Additionally, many countering posts mention 
% an analogy, applying similar logic to an alternate group and state that same reasoning does not generalize. 
These observations point to future directions in generating counterstatements, including tone setting and directly addressing the reader. 
% such as investigations into effects of tone setting and denouncing on users and structure of countering strategies in convincing counterspeech.
% talk more about how the arguments are constructed here

